Fitting tree model with CNN and geodesics to track vesselsand application to Ultrasound Localization Microscopy data

Segmentation of tubular structures in vascular imaging is a well studied task, although it is rare that we try to infuse knowledge of the tree-like structure of the regions to be detected. Our work focuses on detecting the important landmarks in the vascular network (via CNN performing both localization and classification of the points of interest) and representing vessels as the edges in some minimal distance tree graph. We leverage geodesic methods relevant to the detection of vessels and their geometry, making use of the space of positions and orientations so that 2D vessels can be accurately represented as trees. We build our model to carry tracking on Ultrasound Localization Microscopy (ULM) data, proposing to build a good cost function for tracking on this type of data. We also test our framework on synthetic and eye fundus data. Results show that scarcity of well annotated ULM data is an obstacle to localization of vascular landmarks but the Orientation Score built from ULM data yields good geodesics for tracking blood vessels.

==> unused_illustrations/figure_graph.tex <==
\begin{figure}


\begin{subfigure}[b]{0.3\textwidth}
\centering
\begin{tikzpicture}
\node[draw,circle,fill=gray] (P1)at(0,-0.41){1};
\node[draw,circle,fill=gray] (P2)at(0,1){2};
\node[draw,circle,fill=gray] (P3)at(1,-1.41){3};
\node[draw,circle,fill=gray] (P4)at(1,2){4};
\node[draw,circle,fill=gray] (P5)at(2.41,-1.41){5};
\node[draw,circle,fill=gray] (P6)at(2.41,2){6};
\node[draw,circle,fill=gray] (P7)at(3.41,-0.41){7};
\node[draw,circle,fill=gray] (P8)at(3.41,1){8};

\draw[-,very thick,red] (P1) -- (P2);
\draw[-,very thick,red] (P1) -- (P3);
\draw[-,very thick,red] (P1) -- (P4);
\draw[-] (P1) -- (P5);
\draw[-,very thick,red] (P1) -- (P6);
\draw[-] (P1) -- (P7);
\draw[-] (P1) -- (P8);

\draw[-,very thick,red] (P2) -- (P3);
\draw[-,very thick,red] (P2) -- (P4);
\draw[-] (P2) -- (P5);
\draw[-,very thick,red] (P2) -- (P6);
\draw[-] (P2) -- (P7);
\draw[-] (P2) -- (P8);

\draw[-,very thick,red] (P3) -- (P4);
\draw[-] (P3) -- (P5);
\draw[-,very thick,red] (P3) -- (P6);
\draw[-] (P3) -- (P7);
\draw[-] (P3) -- (P8);

\draw[-] (P4) -- (P5);
\draw[-,very thick,red] (P4) -- (P6);
\draw[-] (P4) -- (P7);
\draw[-] (P4) -- (P8);

\draw[-] (P5) -- (P6);
\draw[-,very thick,red] (P5) -- (P7);
\draw[-,very thick,red] (P5) -- (P8);

\draw[-] (P6) -- (P7);
\draw[-] (P6) -- node[right] {$d(x,y)$} (P8);

\draw[-,very thick,red] (P7) -- (P8);
\end{tikzpicture} 
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
\centering
\begin{tikzpicture}
\node[draw,circle,fill=gray] (P1)at(0,-0.41){1};
\node[draw,circle,fill=gray] (P2)at(0,1){2};
\node[draw,circle,fill=gray] (P3)at(1,-1.41){3};
\node[draw,circle,fill=gray] (P4)at(1,2){4};
\node[draw,circle,fill=gray] (P5)at(2.41,-1.41){5};
\node[draw,circle,fill=gray] (P6)at(2.41,2){6};
\node[draw,circle,fill=gray] (P7)at(3.41,-0.41){7};
\node[draw,circle,fill=gray] (P8)at(3.41,1){8};

\draw[-,very thick,blue] (P1) -- (P2);
\draw[-,very thick,blue] (P1) -- (P3);
\draw[-,very thick,red] (P1) -- (P4);
\draw[-] (P1) -- (P5);
\draw[-,very thick,red] (P1) -- (P6);
\draw[-] (P1) -- (P7);
\draw[-] (P1) -- (P8);

\draw[-,very thick,red] (P2) -- (P3);
\draw[-,very thick,red] (P2) -- (P4);
\draw[-] (P2) -- (P5);
\draw[-,very thick,red] (P2) -- (P6);
\draw[-] (P2) -- (P7);
\draw[-] (P2) -- (P8);

\draw[-,very thick,blue] (P3) -- (P4);
\draw[-] (P3) -- (P5);
\draw[-,very thick,blue] (P3) -- (P6);
\draw[-] (P3) -- (P7);
\draw[-] (P3) -- (P8);

\draw[-] (P4) -- (P5);
\draw[-,very thick,red] (P4) -- (P6);
\draw[-] (P4) -- (P7);
\draw[-] (P4) -- (P8);

\draw[-] (P5) -- (P6);
\draw[-,very thick,blue] (P5) -- (P7);
\draw[-,very thick,red] (P5) -- (P8);

\draw[-] (P6) -- (P7);
\draw[-] (P6) -- node[right] {$d(x,y)$} (P8);

\draw[-,very thick,blue] (P7) -- (P8);
\end{tikzpicture} 
\end{subfigure}

\caption{Visualization of the 2 steps on a $8-$complete graph : in the first step we separate clusters of points (in red), an then we find the minimu spanning tree in each connected component (in blue).}
\end{figure}
